Federated Learning of Neural ODE Models with Different Iteration Counts

Federated learning is a distributed machine learning approach in which clients train models locally with their own data and upload them to a server so that their trained results are shared between them without uploading raw data to the server. There are some challenges in federated learning, such as communication size reduction and client heterogeneity. The former can mitigate the communication overheads, and the latter can allow the clients to choose proper models depending on their available compute resources. To address these challenges, in this paper, we utilize Neural ODE based models for federated learning. The proposed flexible federated learning approach can reduce the communication size while aggregating models with different iteration counts or depths. Our contribution is that we experimentally demonstrate that the proposed federated learning can aggregate models with different iteration counts or depths. It is compared with a different federated learning approach in terms of the accuracy. Furthermore, we show that our approach can reduce communication size by up to 92.4% compared with a baseline ResNet model using CIFAR-10 dataset.

==> Makefile <==

# Makefile

LATEX   = platex
BIBTEX  = pbibtex
DVIPS   = dvips
DVIPDF  = dvipdfmx
TARGET  = main
TEXFILE = $(TARGET).tex \
	refer.bib \
	settings.tex \
	abst.tex \
	intro.tex \
	related.tex \
	design.tex \
	eval.tex \
	conc.tex

all: $(TARGET).dvi

dvi: $(TARGET).dvi
$(TARGET).dvi: $(TEXFILE)
	$(LATEX) $(TARGET)
	#$(BIBTEX) $(TARGET)
	#$(LATEX) $(TARGET)
	$(LATEX) $(TARGET)

ps: $(TARGET).ps
$(TARGET).ps: $(TARGET).dvi
	$(DVIPS) -f $(TARGET).dvi > $(TARGET).ps

pdf: $(TARGET).pdf
$(TARGET).pdf: $(TARGET).dvi
	$(DVIPDF) $(TARGET).dvi

clean:
	rm -f $(TARGET).dvi
	rm -f $(TARGET).ps
	rm -f $(TARGET).log
	rm -f $(TARGET).out
	rm -f $(TARGET).pdf
	#rm -f $(TARGET).bbl
	rm -f $(TARGET).blg
	rm -f *.aux *~ 


